Asymptotically-Optimal Motion Planning using Lower Bounds on Cost

Many path-finding algorithms on graphs such as A* are sped up by using a heuristic function that gives lower bounds on the cost to reach the goal. Aiming to apply similar techniques to speed up sampling-based motion-planning algorithms, we use effective lower bounds on the cost between configurations to tightly estimate the cost-to-go. We then use these estimates in an anytime asymptotically-optimal algorithm which we call Motion Planning using Lower Bounds (MPLB). MPLB is based on the Fast Marching Trees (FMT*) algorithm recently presented by Janson and Pavone. An advantage of our approach is that in many cases (especially as the number of samples grows) the weight of collision detection in the computation is almost negligible with respect to nearest-neighbor calls. We prove that MPLB performs no more collision-detection calls than an anytime version of FMT*. Additionally, we demonstrate in simulations that for certain scenarios, the algorithmic tools presented here enable efficiently producing low-cost paths while spending only a small fraction of the running time on collision detection.

==> tex/lbt_fmt.tex <==
\section{Lower Bound Tree FMT*}
\label{sec:lbt}
We suggest to apply the concepts suggested in the work on LBT-RRT~\cite{SH13} to the FMT* algorithm and note that this can be applied both to aFMT* and to \LB.
For ease of exposition we describe the tool applied to aFMT* (see Algorithm~\ref{alg:near_optimal_fmt}) and call this variant LBT-FMT*. 
The application to \LB is then a fairly straightforward extension.
We suggest to compute an \emph{asymptotically near-optimal} solution by constructing two trees simultaneously.
The first tree \Tlb stores a \emph{lower bound} on the cost to reach each node while the second tree, \Tapx stores an approximation of the cost to reach each node.
At every stage of the algorithm we will maintain the following invariants:

\begin{enumerate}
	\item \textbf{Bounded approximation invariant\footnote{The bounded approximation invariant presented in the appendix is not to be confused with the bounded approximation invariant used for the \LB algorithm. We use the same name to be consistent with~\cite{SH13}.}}\\
				For each node $x \in \Tlb, \Tapx$, 
				$\texttt{cost-to-go}_{\Tapx}(x) 
					\leq 
				(1 + \varepsilon) \cdot \texttt{cost-to-go}_{\Tlb}(x)$.
	\item \textbf{Lower bound invariant}\\
				For each node $x \in \Tlb$, 
				$\texttt{cost-to-go}_{\Tlb}(x) 
					\leq 
				 \texttt{cost-to-go}_{\texttt{FMT}^*}(x)$ 
				after $x$ is in the tree of the FMT* algorithm, which was run on the 
				same set of nodes.
\end{enumerate}


\begin{algorithm}[ht]
\caption{LBT-FMT* (Cache)}
\label{alg:near_optimal_fmt}
\begin{algorithmic}[1]
	\STATE	$V \leftarrow \set{x_{init}} \cup \texttt{sample\_free}(n)$;
					\hspace{3mm}
					$E \leftarrow \emptyset$
  \STATE	$W \leftarrow V \setminus \set{x_{init}}$;
  				\hspace{3mm}
					$H \leftarrow \set{x_{init}}$
					\hspace{3mm}
					// \textsf{$H$ is ordered according to $\texttt{cost}_{\Tlb}$}
  \FORALL{$v \in V$} 
  	\STATE	$N_v \leftarrow 
  					\texttt{nearest\_neighbors}(V \setminus \set{v}, v, r_n)$
  \ENDFOR
  
%  \vspace{2mm}

  \STATE	$z \leftarrow x_{init}$
	\WHILE {$z \notin \calX_{Goal}	$}
		\STATE $H_{new} \leftarrow \emptyset$
		\STATE $X_{near} \leftarrow W \cap N_z$
						\hspace{3mm}
						// \textsf{nearest vertices of $z$ not in roadmap }
		
	  \vspace{2mm}

		\FOR  {$x \in X_{near}$}
			\STATE $Y_{near} \leftarrow H \cap N_x$
							\hspace{3mm}
							// \textsf{nearest vertices of $x$ in roadmap}
			\STATE $y_{min\ lb} \leftarrow \arg \min_{y \in Y_{near}} 
								\set{\texttt{cost-to-go}_{\Tlb}(y) + \texttt{cost}(y,x)} $
			\STATE $y_{min\ apx} \leftarrow \arg \min_{y \in Y_{near}} 
								\set{\texttt{cost-to-go}_{\Tapx}(y) + \texttt{cost}(y,x) $ 
								and 
								$\texttt{collision\_free\_using\_cache}(y, x) } $
		
			\vspace{2mm}
		
			\IF {$\texttt{cost-to-go}_{\Tapx}(y_{min\ apx}) + 
						\texttt{cost}(y_{min\ apx},x) 
							\leq 
					 (1+\varepsilon) \cdot 
					 (\texttt{cost-to-go}_{\Tlb}(y_{min\ lb}) + 
					 \texttt{cost}(y_{min\ lb}, x))$}
				\STATE $\Tlb.\texttt{parent}(x) \leftarrow y_{min\ lb}$
				\STATE $\Tapx.\texttt{parent}(x) \leftarrow y_{min\ apx}$
			
				\STATE $H_{new} \leftarrow H_{new} \cup \set{x}$
							 \hspace{3mm}
							 $W \leftarrow W \setminus \set{x}$
				
			\ELSE
				\IF {\texttt{collision\_free}$(y_{min\ lb}, x)$}
					\STATE $\Tlb.\texttt{parent}(x) \leftarrow y_{min\ lb}$
					\STATE $\Tapx.\texttt{parent}(x) \leftarrow y_{min\ lb}$
				
					\STATE $H_{new} \leftarrow H_{new} \cup \set{x}$
							 	 \hspace{3mm}
							   $W \leftarrow W \setminus \set{x}$					
				\ENDIF
			\ENDIF
		\ENDFOR
		
		\vspace{2mm}
					
		\STATE $H \leftarrow (H \cup H_{new}) \setminus \set{z}$
		\IF {$H = \emptyset$}
			\RETURN FAILURE
		\ENDIF
		
		\STATE $z \leftarrow \arg \min_{y \in H} 
								\set{\texttt{cost}(y)} $
						
	\ENDWHILE

	\RETURN PATH 
\end{algorithmic}
\end{algorithm}						

The Bounded approximation invariant is maintained by construction (using a proof similar to the one presented in~\cite{SH13}).
Let us note several straightforward (yet helpful) observations:

\begin{obs}
	The set of nodes of \Tlb and \Tapx are identical at every stage of the algorithm.
\end{obs}

\begin{obs}
	Every edge of \Tapx is collision free.
\end{obs}

Now,
\begin{lem}
	The Lower bound invariant is maintained by LBT-FMT*
\end{lem}
\begin{proof}
The proof is by induction on the nodes in $H$ where the base trivially holds for $x_{init}$.
Now, for the induction step,
assume that for every node in $H$ the lower bound invariant holds.
Let $z$ be the node with the lowest cost in $H$ (i.e., the node with the lowest cost in \Tlb).
As the induction hypothesis holds we know that 
$\texttt{cost-to-go}_{\Tlb}(z) \leq \texttt{cost-to-go}_{FMT^*}(z)$ after $z$ is in the tree of the FMT* algorithm run on the same set of nodes.

Recall that 
$X_{near} \leftarrow W \cap N_z$ is the set of nearest vertices of $z$ not in the  search tree and that for each such $x$,
$Y_{near} \leftarrow H \cap N_x$ is the set of nearest vertices of $x$ in the search tree.
We show for every $x \in X_{near}$ that if it is added to $H$ then the lower bound invariant is maintained for $x$ namely,
$\texttt{cost-to-go}_{\Tlb}(x) \leq \texttt{cost-to-go}_{FMT^*}(x)$.

If $x$ is added to $H$ then 
\[
	\texttt{cost-to-go}_{\Tlb}(x) 
		= 
 	\texttt{cost-to-go}_{\Tlb}(y_{min\ lb}) + 
 	\texttt{cost}(y_{min\ lb}, x)
\]
where
\[
	y_{min\ lb} = \arg \min_{y \in Y_{near}} 
								\set{\texttt{cost-to-go}_{\Tlb}(y) + \texttt{cost}(y, x)}. 
\]
There exists a node $z' \in Y_{near} $ such that \\
$\texttt{cost-to-go}_{\Tlb}(z) \leq \texttt{cost-to-go}_{\Tlb}(z')$
and 
$\texttt{cost-to-go}_{\text{FMT*}}(x) 
		= 
 \texttt{cost-to-go}_{FMT*}(z') + 
 \texttt{cost}(z', x)$.\\
Now, 
\begin{align*}
	\texttt{cost-to-go}_{\Tlb}(x) 
	& =
	\texttt{cost-to-go}_{\Tlb}(y_{min\ lb}) + 
 	\texttt{cost}(y_{min\ lb}, x) \\
	& \leq
	\texttt{cost-to-go}_{\Tlb}(z') + 
 	\texttt{cost}(z', x) \\ 	
	& \leq 
	\texttt{cost-to-go}_{\text{FMT*}}(z') + 
 	\texttt{cost}(z', x) \\
 	& =
	\texttt{cost-to-go}_{\text{FMT*}}(x). 	
\end{align*}



%\[
%	\texttt{cost-to-go}_{\Tlb}(x) 
%		= 
%	\texttt{cost-to-go}_{\Tlb}(y_{min\ lb}) + 
% 	\texttt{cost}(y_{min\ lb}, x)
% 		\leq
% 	\texttt{cost-to-go}_{\Tlb}(z') + 
% 	\texttt{cost}(z', x) 
% 		\leq
% 	\texttt{cost-to-go}_{\text{FMT*}}(z') + 
% 	\texttt{cost}(z', x)
% 		=
% 	\texttt{cost-to-go}_{\text{FMT*}}(x)
%\]
 Where the first equality  is by the behavior of the algorithm (line 14 or line~19),
 the first inequality comes from the fact that $y_{min\ lb}$ attains the minimum over $Y_{near}$ and the second inequality comes from the induction hypothesis.
\end{proof}

Note that this technique is general for any cached information maintained by  the algorithm.
Specifically, we use the cache provided by previous iterations.

%\section{Thoughts, ToDo etc.}
%In some scenarios each node will be connected to its ancestor. In this case we only save one call to the local planner per \textbf{node in the previous iteration}.
%For every newly sampled node \textbf{the cache is not used} thus the speedup will probably be very small.
%
%To overcome this one needs to look into two lines of research\\
%(1)~In which scenarios will the cache be most beneficial?
%(2)~How can the LB-technique be applied to \textbf{newly introduced nodes}.
%This may be done by:
%(2.1)~methods similar to Bialkowski et al.~\cite{BKOF12} or 
%(2.2)~by exploiting the observation that as the radius shrinks the probability that a node will be connected to each neighbor tends to one.
%Here, one may not consider new nodes unless the pose a significant advantage over the LBT coast and or the APX cost.
%
%We need to solve the problem that each new node that is close to an old node (hence not changing the solution by much) is checked for collision detection (as the cache is empty).
%(2.1) solves this but is not applicable to non-Euclidean spaces.
%We should try to use the lower bound as an alternative.
%
%For scenarios consider a scenario scattered with small obstacles which will make the exact solution do a lot of work refining the solution while the apx solution will not waste time until the improvement is substantional.
%
%Should we cache distances?
%
%at least cut by half the number of nn computations
%
%If we want to further reduce local planning cost (although this may be unnecessary) we can follow the following scheme:
%For each sample that does not have an approximate cost (apx costs from previous iterations are not thrown away until a new value comes), and that is revealed, we record the lower bound to reach this edge as the distance from bet node in $H$ (now we do not maintain the bounded approximation invariant).
%We continue our search on the nodes.
%If a node is revealed and its best parent is a node with no apx cost then we have two cases:\\
%(i) the node does not have an apx cost or \\
%(ii) the node has an apx cost.
%
%If the node does not have an apx cost, then we continue recursively.
%If the node has an apx cost, again we look into two cases: \\ 
%(a) the bounded approximation invariant is maintained (and we continue normally) or \\
%(b) the bounded approximation invariant is violated.
%In this case we need to do local planning and a possible rollback: i.e. we go to ancestors until we find the first that has apx cost and start doing local planning.
%




==> tex/regular_obs.tex <==
\section{Theoretical Analysis}
Let $B(x,r)$ denote the ball centered at $x$ of radius $r$.
A region $\calX$ is said to be \emph{regular} if there exists $\xi > 0$ such that $\forall y \in \partial \calX$, there exists $z \in \calX$ such that $B(z, \xi ) \in \calX$ and $y \in B(z, \xi )$. 
In other words, a regular region is a "well-behaved" set where the boundary has bounded curvature.
We will say that a region $\calX$ is $\xi$-regular if $\calX$ is regular for the parameter $\xi$.

%Assume that each obstacle is $\xi$-regular and consider two configurations $p,q \in \Cfree$ such that $pq \notin \Cfree$ and $|pq| \leq 2 \xi$.
%We want to bound:\\
%\begin{enumerate}
%	\item The length of the collision-free path connecting $p$ and $q$
%	\item The probability that such an event occurs.	
%\end{enumerate}

%We start with the analysis in $\R^2$.

%Now, given a node $x$ in a roadmap produced by the FMT* algorithm in the $i$'th iteration, 
%let $f_i(x)$ denote the cost-to-come to reach the node from the start location and let $h_i(x)$ denote the cost-to-go to reach the goal node from $x$ computed as the shortest path in the neighborhood graph produced by considering a connection radius of $r(N_i)$ where $N_i$ is the number of nodes in the $i$'th iteration.
%
%If $f_i(x) + h_i(x) \leq (1 + \varepsilon) f_{i-1}(x_{goal})$ then there may exist a path which is much better than the existing one.
%What is the probability that this is NOT the case.
%I.e. what is the probability that we expand a node that may not be useful?
%If $r(N_i) \leq 2\xi$ then this is zero!

\begin{lem}
	If the obstacle-space, \Cforb, consists of $\xi$-regular obstacles, 
	then for each two collision-free configurations $p,q, \in \Cfree$ such that
	$|pq| \leq 2 \xi$, 
	the length $|P(p,q)|$ of the shortest collision-free path connecting $p$ and 
	$q$ is 
	bounded by $\frac{\pi}{2} |pq|$.
\end{lem}

\begin{proof}
If $pq \in \Cfree$, then clearly $|P(p,q)| = |pq|$ and the bound is $1 \leq \frac{\pi}{2}$

If not, then $pq \notin \Cfree$ and the two configurations intersect an obstacle which is regular.
Locally, the obstacle looks like a ball and roughly speaking, the worst case can happen when $p$ and $q$ are exactly on opposite sides of the ball, i.e.  $|pq| = 2 \xi$. In this case a path in the free space will have to travel along the boundary of the ball which is of distance $\pi \xi$.
Hence, the ratio between the collision-free path connecting $p$ and $q$ and $|pq|$ is:
\[
	\frac{|\text{Path}(p,q)|}{|pq|}  \leq \frac{\pi \xi}{2 \xi} = \frac{\pi}{2}
\]
Thus
\[
	|\text{Path}(p,q)| \leq \frac{\pi}{2} |pq|
\]

This ratio may not be attained by vertices in the current graph but it is a bound on the possible path connecting $p$ and $q$.
\end{proof}

Thus immediately we can conclude the following corollary:
\begin{cor}
	If the obstacle-space, \Cforb, consists of $\xi$-regular obstacles, 
	and $r(n) \leq 2 \xi$ ($r(n)$ is the connection radius)
	then for every configuration $x \in \Cfree$ 
	such that there exists a path between $x$  
	and $x_{goal}$ in the neighborhood graph it holds that 
	$P_{free} (x, x_{goal} \leq) \frac{\pi}{2} \cdot P_{G_n} (x, x_{goal})$
	configuration $x$
	then for each two collision-free configurations $p,q, \in \Cfree$ such that
	$|pq| \leq 2 \xi$, 
	the length $|P(p,q)|$ of the shortest collision-free path connecting $p$ and 
	$q$ is 
	bounded by $\frac{\pi}{2} |pq|$.
\end{cor}

Now, consider a configuration space where the obstacle-space, \Cforb, consists of $\xi$-regular obstacles and we have two paths $P_1, P_2$ fro the source to the goal configuration such that:\\
\begin{enumerate}
	\item The length of $P_1, P_2$ denoted by $l_1, l_2$ is such that
				$l_1 = a l_2$ for some large $a$.
	\item The clearance of $P_1, P_2$ denoted by $\gamma_1, \gamma_2$ is such 
				that
				$\gamma_2 = b \gamma_2$ for some large $b$.
\end{enumerate}

Assume that $\gamma_2$ is large, finding a path in the homotopy class of $P_2$ is easy.
Once such a solution is found 

==> tex/visualization.tex <==
\section{Visualization of aFMT* and \LB}
\label{sec:visualization}
\textVersion
{We consider a point robot moving in the plane and run aFMT* and \LB for four iterations using $50*2^i$ samples in the $i$'th iteration.}
{To further clarify the behavior of aFMT* and \LB we consider a point robot translating in the plane.
We run both algorithms for four iterations using $50*2^i$ samples in the $i$'th iteration.}
The setting contains one obstacle within a square room and
source and target configurations located at the upper left and lower left corners of the square, respectively.
\textVersion
{
Figure~\ref{fig:lb} depicts 
the disk graph $\calG_i$ for each iteration, the search-tree of aFMT* and the search-tree of \LB.
}
{
Bypassing the obstacle in a clockwise fashion is easy as there are paths with high clearance while 
bypassing the obstacle in a counterclockwise fashion is much harder due to the low clearance along such paths.

%Figures~\ref{fig:neighberhoods},~\ref{fig:fmt} and~\ref{fig:lb} depict
Figure~\ref{fig:lb} depicts 
the disk graph $\calG_i$ for each iteration, the search-tree of aFMT* and the search-tree of \LB.
%, respectively.
}

\begin{figure*}[h]
\vspace{-5mm}
  \centering
  \subfloat
   [\sf 50 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/DG__Iteration_0_50_samples.png}
   	\label{fig:neighberhood0}
   }
   \hspace{1mm}
  \subfloat
   [\sf 100 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/DG__Iteration_1_100_samples.png}
   	\label{fig:neighberhood1}
   }
   \hspace{1mm}
  \subfloat
   [\sf 200 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/DG__Iteration_2_200_samples.png}
   	\label{fig:neighberhood2}
   }
   \hspace{1mm}
  \subfloat
   [\sf 400 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/DG__Iteration_3_400_samples.png}
   	\label{fig:neighberhood3}
   }\\
  \subfloat
   [\sf 50 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_0_50_samples_epsilon_00.png}
   	\label{fig:fmt0}
   }
   \hspace{1mm}
  \subfloat
   [\sf 100 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_1_100_samples_epsilon_00.png}
   	\label{fig:fmt1}
   }
   \hspace{1mm}
  \subfloat
   [\sf 200 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_2_200_samples_epsilon_00.png}
   	\label{fig:fmt2}
   }
   \hspace{1mm}
  \subfloat
   [\sf 400 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_3_400_samples_epsilon_00.png}
   	\label{fig:fmt3}
   }\\   
  \subfloat
   [\sf 50 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_0_50_samples_epsilon_02.png}
   	\label{fig:lb0}
   }
   \hspace{1mm}
  \subfloat
   [\sf 100 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_1_100_samples_epsilon_02.png}
   	\label{fig:lb1}
   }
   \hspace{1mm}
  \subfloat
   [\sf 200 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_2_200_samples_epsilon_02.png}
   	\label{fig:lb2}
   }
   \hspace{1mm}
  \subfloat
   [\sf 400 samples]
   { 
   	\includegraphics[height =2.65 cm]{pics/Tight_w_corridors/FMT_tree__Iteration_3_400_samples_epsilon_02.png}
   	\label{fig:lb3}
   }   
  \caption{	(a)-(d) the disk graph $\calG_i$, 
  					(e)-(h) aFMT* search-tree using $\calH_i$ and
  					(i)-(l) \LB search tree with $\varepsilon = 0.2$ using $\calH_i$.}
  \vspace{-10mm}
  \label{fig:lb}
\end{figure*}
